Error-Bounded Correction of Noisy Labels

To collect large scale annotated data, it is inevitable to introduce label noise, i.e., incorrect class labels. To be robust against label noise, many successful methods rely on the noisy classifiers (i.e., models trained on the noisy training data) to determine whether a label is trustworthy. However, it remains unknown why this heuristic works well in practice. In this paper, we provide the first theoretical explanation for these methods. We prove that the prediction of a noisy classifier can indeed be a good indicator of whether the label of a training data is clean. Based on the theoretical result, we propose a novel algorithm that corrects the labels based on the noisy classifier prediction. The corrected labels are consistent with the true Bayesian optimal classifier with high probability. We incorporate our label correction algorithm into the training of deep neural networks and train models that achieve superior testing performance on multiple public datasets.

==> theory_ideal.tex <==

\section{Method}

Given training data with corrupted labels, our method has two synchronized modules, the training module and the label correction module. See Figure \ref{fig:overview} for an overview. The label correction module continues to update labels of the training data so that they are likely ``correct'' (the meaning of ``correct'' will be elaborated later). Meanwhile, the training module continues to learn a classifier based on the updated labels. As more labels are corrected, the classifier converges to a desired one, which correctly predicts uncorrupted labels.

Like any other data-re-calibrating method, the major challenge is to control the quality of label correction without knowing the uncorrupted labels. The only available information is the current classifier's prediction, called $f$. Denote by $\eta$ the true conditional distribution of the original (uncorrupted) labels. Denote by $\etanoise$ its counterpart in the noisy (corrupted) label setting. 
Our main insight is a closed form relationship between $\eta$ and $\etanoise$ when the label noise is i.i.d.~distributed.
Since $f$ essentially approximates $\etanoise$, we prove that when $f$ dominantly predicts that a datum has a particular label, $y$, it is highly possible that $y$ is the clean label of this datum.

uses $f$ for a likelihood ratio test. Based on the test result, it decides whether to correct the label of a datum. Our main theorem (Thm \ref{thm:lrt}) states that the algorithm will change the labels to the correct ones, i.e., the ones consistent with the Bayes optimal classifier.

 We incrementally train a deep neural network based on the corrected labels, $\ynoise$. Meanwhile, the network's prediction is used for label correction. To improve the quality of the prediction, we introduce a new loss term, called the \emph{retroactive loss}. The goal is to regulate the model using models trained in earlier epoches, as they may be less overfitting with corrupted labels. 

 For the label correction module, we focus on a binary classifier. But the algorithm and the theoretical results can easily be generalized to the multiclass setting (Corollary \ref{cor:multiclass}).

We start with some preliminaries necessary for the exposition (Section \ref{sec:prelim}).
In Section \ref{sec:correction}, we explain our correction algorithm. 
In Section \ref{sec:dnn-training}, we present the overall  training method.

\begin{figure}[bt!]
\begin{center}
\includegraphics[width=.3\textwidth]{figs/Overview.pdf}
\caption{The overview of our method.}
\label{fig:overview}
\end{center}
\end{figure}

\subsection{Preliminaries}
\label{sec:prelim}

Let $\mathcal{X}$ be the feature space, $\mathcal{Y}=\{0,1\}$ be the label space, and $D$ be an unknown distribution on $\mathcal{X} \times \mathcal{Y}$. The joint probability can be factored as $D(\vx,y) = \pr(y|\vx)\pr(\vx)$. We denote by $\eta_y(\vx) = \pr(y \mid \vx)$ the \emph{true conditional probability}. 
The \emph{Bayes risk} of a classifier $h:\gX\rightarrow \gY$ is $R(D,h) = \Pr_{(\vx,y) \sim D} (h(\vx) \neq y)$.
A \emph{Bayes optimal classifier} is the minimizer of the Bayes risk, i.e., \mbox{$h^\ast = \argmin_h R(D,h)$}. 
It can be calculated using the true conditional probability, $\eta$,
\begin{align}
    h^*(\vx) = 
    \sI_{ \left\{\eta_1(\vx)\geq\frac{1}{2} \right\}}(\mathbf{x}) = 
    \left\{
        \begin{array}{cl}
        1 & \text{if}\quad \eta_1(\vx) >= \frac{1}{2}\\
        0 & \text{otherwise}
        \end{array}.
    \right.
\end{align}

We assume the true conditional probability, $\eta$, satisfies the Tsybakov condition (also called the TNC condition) \citep{tsybakov2004optimal}. This condition, also called margin assumption, stipulates that the uncertainty of $\eta$ (region close to decision boundary at $1/2$) and thus the Bayes optimal classifier is bounded. 

\begin{definition}[Tsybakov Condition] There exist $C>0,\lambda>0$, and $t_0 \in (0, \frac{1}{2}]$, such that for all $t \leq t_0$, 
$$\Pr\left[ \left| \eta_1(\vx) - \frac{1}{2} \right| < t \right] \leq Ct^\lambda.$$ 
\end{definition}

\textbf{The noisy label setting.}
Instead of samples from $D$, we are given a sample set with noisy labels
$\mathcal{S}=\{(\vx,\widetilde{y})\}$ 
where $\ynoise$ is the possibly corrupted label based on the true label $y$. We assume a \emph{transition probability} $\tau_{i\rightarrow j} = \pr(\widetilde{y}=j | y=i)$, i.e., the chance a ground truth label $y$ is flipped from class $i$ to class $j$. For simplicity, we denote $\tau_{ij}=\tau_{i\rightarrow j}$. 
The transition probabilities $\tau_{01}$ and $\tau_{10}$ are independent of the true joint distribution $D$ and the feature $\vx$. 
We denote the conditional probability of the noisy labels as $\widetilde{\eta}_1(\vx) = \pr(\widetilde{y}=1 | \vx)$. In short, we call $\widetilde{\eta}$ the \emph{noisy conditional probability}. It is related linearly to the true conditional probability, $\eta$: 
\begin{align*}
\widetilde{\eta}_1(\vx) 
&= (1-\tau_{10})\eta_1(\vx) + \tau_{01}[1-\eta_1(\vx)] \\
&= (1-\tau_{01}-\tau_{10})\eta_1(\vx) + \tau_{01}.
\label{eq:etanoise}
\end{align*}

\subsection{The Label Correction Algorithm and its Theoretical Guarantees} 
\label{sec:correction}

Our label correction algorithm takes in a current neural network prediction $f:\mathcal{X}\rightarrow [0,1]$ (i.e., an estimation of $\eta$ based on the noisy labels). For all training data and their current noisy label $(\vx,\ynoise)$, the correction algorithm uses $f$ to run a likelihood ratio test and to decide whether to flip the label according to the result. 
The goal of the likelihood test is to decide whether the null hypothesis, $H_0 : \ynoise=y$, is true. If yes, $\ynoise$ is accepted as it is. Otherwise, we flip $\ynoise$, so that hopefully it becomes $y$.
Formally, the likelihood ratio is defined as 
\begin{equation}
\LR(f,\vx,\ynoise) = \frac{f(\vx)^{\widetilde{y}}\left[1-f(\vx)\right]^{1-\widetilde{y}}}{f(\vx)^{1-\widetilde{y}}\left[1-f(\vx)\right]^{\widetilde{y}}}.
\label{eq:lr}
\end{equation}
We compare this likelihood ratio with a predetermined value $\Delta$. If $\LR(f,\vx,y)\leq \Delta$, we reject the null hypothesis and flip the label $\ynoise_{new} = 1-\ynoise$. Otherwise, the label remains unchanged, $\ynoise_{new} = \ynoise$.
See Figure \ref{fig:synth} for an illustration of the algorithm.

\begin{figure*}[tbp]
\centering
\begin{tabular}{cc}
    \includegraphics[width=.48\textwidth]{figs/Fx.png} &
    \includegraphics[width=.48\textwidth]{figs/Eta_for_LRT.png} \\
    (a) Noisy labels and $f$. & (b) Corrected labels and $\eta$.  \\
    \includegraphics[width=.48\textwidth]{figs/LR_for_One.png} &
    \includegraphics[width=.48\textwidth]{figs/LR_for_Zero.png} \\
    (c) $\LR$ for $\ynoise=1$. & (d) $\LR$ for $\ynoise=0$.
\end{tabular}
    \caption{An illustration of the label correction algorithm. $\Delta$ is set to 1. (a): a corrupted sample and its corresponding classifier prediction $f$. (b): after correction, the labels are consistent with the true conditional probability, $\eta$. (c): likelihood ratio for $\ynoise=1$. Data with $x<0$ are corrected to $\etanoise_{new}=0$ as $LR(\vx)$ are below $\Delta=1$. (d): likelihood ratio for $\ynoise=0$. Data with $x>0$ are corrected to $\etanoise_{new}=1$ as $LR(\vx)$ are below $\Delta=1$.}
    \label{fig:synth}
\end{figure*}

Note that the constant $\Delta$ depends on the underlying noise pattern and $f$. 
Below we show that if we choose $\Delta$ carefully, the label correction algorithm is guaranteed to make proper correction and clean most of the corrupted labels. However, in practice, $\Delta$ is unknown and needs to be tuned. 

\textbf{Intuition.} In the likelihood ratio (Eq.~(\ref{eq:lr})), the numerator is the likelihood that the prediction $f$ is consistent with the noisy label $\ynoise$. The denominator is the likelihood of the opposite case.
When this ratio is smaller than $1$, we know that the prediction of $f$ is more likely to be inconsistent with $\ynoise$. But whether $f$ agrees with $\ynoise$ is not the hypothesis to test.
To test the intended null hypothesis ($\ynoise = y$), we need to check whether $\ynoise$ is consistent with the true conditional distribution $\eta$, namely, the Bayes optimal classifier prediction $h^\ast(\vx)$. To this end, we assume $f$ is a close enough approximate of $\etanoise$ as it is trained on the noisy labels. 
This way, testing whether $f$ agrees with $\ynoise$ is close to testing whether $\etanoise$ agrees with $\ynoise$, except that the threshold $\Delta$ needs to be carefully chosen. Another issue we need to consider is that the $\Delta$ is unknown. Our main theorem will bound the chance of failed correction by how close $f$ approximates $\etanoise$ and how close we can set $\Delta$ to the perfect one.

\subsubsection{Formal Statement of the Algorithm and the Theorem}

Assume the knowledge of some prediction function $f$ (perhaps from a neural network). The label correction algorithm is given in Procedure 1. It checks the likelihood ratio with regard to a parameter $\Delta = \min (\frac{1+\tau_{01}-\tau_{10}}{1+\tau_{10}-\tau_{01}}, \frac{1+\tau_{10}-\tau_{01}}{1+\tau_{01}-\tau_{10}})$. If $\LR$ is no greater than $\Delta$, we flip the label. Otherwise, $\ynoise_{new}$ is the same as $\ynoise$. Note that one only needs to know the difference $\tau_{01}-\tau_{10}$ in order to know $\Delta$. In practice, $\Delta$ may be unknown and needs to be decided empirically.

\begin{table}[h]
\centering
\begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\texttt{LRT-Correction}}\label{alg:LRT}
\begin{algorithmic}[1]
\REQUIRE $(\vx, \widetilde{y}), f(\vx), \Delta$.
\ENSURE $\widetilde{y}_{new}$
\IF{$\LR(f,\vx,\ynoise) \leq \Delta$}
\STATE $\widetilde{y}_{new} = 1-\widetilde{y}$
\ELSE 
\STATE $\widetilde{y}_{new} = \widetilde{y}$
\ENDIF
\end{algorithmic}
\end{algorithm}
\end{minipage}
~
\begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\texttt{LRT-MultiCorrection}}\label{alg:LRT}
\label{multialgorithm}
\begin{algorithmic}[1]
\REQUIRE $(\vx, \ynoise), f(\vx), \Delta$.
\ENSURE $\widetilde{y}_{new}$

$y*:=\argmax_{i} [f(\vx)]_{i}$;
$\LR(f,\vx,\ynoise):= \frac{[f(\vx)]_{\widetilde{y}}}{[f(\vx)]_{y*}}$;
\IF {$\LR(f,\vx,\ynoise) \leq \Delta$}
\STATE $\widetilde{y}_{new} = y*$
\ELSE 
\STATE $\widetilde{y}_{new} = \widetilde{y}$
\ENDIF
\end{algorithmic}
\end{algorithm}
\end{minipage}
~~~ 
\end{table}

Our main theorem states that suppose the classifier prediction, $f$, is a close approximation of the noisy conditional probability, $\etanoise$. And suppose we can find a good enough $\Delta^{'}$ that is close enough to the ideal $\Delta$. Then there is a very good chance that our algorithm corrects most labels to the correct ones, i.e., the same as the Bayes optimal classifier prediction. Please note that here ``proper correction'' means that the new label, $\ynoise_{new}$, is the same as the Bayes optimal classifier prediction, $h^\ast(\vx)$, instead of $y$. This is well justified as it means that the correction will give us a classifier as good as the Bayes optimal one.

\sz{I made change to the notation to all previous section such that I don't have restate here. And Corollary 1 is added at the end of the theory ideal section. Corollary 2 and 3 are added at the end of theory practice section}

\begin{theorem}
\label{thm:main}
\label{epsilontheorem}

Assume $\eta(\vx)$ satisfies the Tsybakov condition with constants $C>0$ and $\lambda>0$. Let $h^{*}$ denote the Bayes optimal classifier, and $\widetilde{\eta}(\vx)$ the noisy conditional probability, $\widetilde{\eta}_1(\vx) = \Pr(\widetilde{y} = 1 \mid \vx) = (1-\tau_{01}-\tau_{10})\eta_1(\vx)+\tau_{01}$. Let $f$ be any classifier such that $\vert \vert f(\vx) - \widetilde{\eta}(\vx)\vert \vert_{\infty} \leq \epsilon$ for some $\epsilon>0$ , then $\exists \Delta \in (0, 1)$ s.t 
\[\Pr_{(x,y)\sim D} (\ynoise \neq h^*, f \leq \Delta) +  \geq 1 - C \left[ \mathcal{O}(\epsilon) \right]^{\lambda}. \]

for symmetric noise, $\Pr_{(x,y)\sim D} (\ynoise \neq h^* \mid \tau_{01}=\tau_{10}) \geq 1-C\left(\epsilon/2\right)^{\lambda}$.
\end{theorem}

\textbf{Intuition of the proof.} 
We will prove two lemmas. The first lemma shows that when $f$ is linear in $\eta$, i.e., $f(\vx)=a \eta(\vx) + b$, with known coefficients $a,b$, we can find a $\Delta$ such that then the correction algorithm can be correct everywhere. The second lemma proves a more relaxed version. If $f$ is exactly $\etanoise$ and if we only know the difference between the transition probabilities, $\tau_{01}-\tau_{10}$, then we can bound the chance of mistakes of the correction algorithm. Finally, based on these two lemmas, careful case analysis, and the Tsybakov condition of the true conditional probability, $\eta$, we can prove the theorem. The complete proof can be found in supplementary material.

\textbf{Multiclass setting.} So far, all the description and theoretical results are based on a binary classification setting. However, the results can be generalized to a multiclass setting without any technical difficulties. Let $\ynoise$ be the observed (possibly) corrupted label, $f(\vx)$ be a classifier vector, where $[f(\vx)]_{i}$ (the $i$th coordinate of $f(\vx)$) specifies the confidence of assigning $\vx$ to class $i$. The algorithm is presented in Procedure~\ref{multialgorithm}. Informally, we present the theoretical guarantee for multiclass LRT as Corollary \ref{cor:multiclass}. The proof is left for a journal version. 

\begin{corollary}
\label{cor:multiclass}
\textbf{Corollary 1.}
Assume $\widetilde{\eta}_i(\vx) = \Pr(\widetilde{y}=i \mid \vx)$ and fulfills multi-class Tsybakov condition $\Pr\left[\left\lvert \widetilde{\eta}_m(\vx) - \widetilde{\eta}_{\phi}(\vx)\right\rvert \leq t\right] \leq C(t)^\lambda$ for constant $C>0, t>0$. For the noisy conditional probability $\widetilde{\eta}_i(\vx \mid i,j) = (1-\tau_{i,j}-\tau_{j,i})\eta_i(\vx \mid i,j) + \tau_{j,i}$. If we have $\vert \vert f(\vx) - \widetilde{\eta}(\vx)\vert \vert_{\infty} \leq \epsilon$ then $\exists \Delta > 0$ s.t:
\[\Pr_{(x,y)\sim D} (\ynoise = h^*(\vx), f_{\ynoise}(\vx) < \Delta) \leq C\left[O(\epsilon)\right]^\lambda \]\\
\end{corollary}

